Towards an Understanding of the Correlations in Jet Substructure

Over the past decade, a large number of jet substructure observables have been proposed in the literature, and explored at the LHC experiments. Such observables attempt to utilize the internal structure of jets in order to distinguish those initiated by quarks, gluons, or by boosted heavy objects, such as top quarks and W bosons. This report, originating from and motivated by the BOOST2013 workshop, presents original particle-level studies that aim to improve our understanding of the relationships between jet substructure observables, their complementarity, and their dependence on the underlying jet properties, particularly the jet radius and jet transverse momentum. This is explored in the context of quark/gluon discrimination, boosted W boson tagging and boosted top quark tagging.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = boost2013_report

default: pdflatex

nobibtex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}


testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

pdflatex:
	make clean
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

pdflatexnobibtex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


